Adapting by Analogy: OOD Generalization of Visuomotor Policies via Functional Correspondence

End-to-end visuomotor policies trained using behavior cloning have shown a remarkable ability to generate complex, multi-modal low-level robot behaviors. However, at deployment time, these policies still struggle to act reliably when faced with out-of-distribution (OOD) visuals induced by objects, backgrounds, or environment changes. Prior works in interactive imitation learning solicit corrective expert demonstrations under the OOD conditions -- but this can be costly and inefficient. We observe that task success under OOD conditions does not always warrant novel robot behaviors. In-distribution (ID) behaviors can directly be transferred to OOD conditions that share functional similarities with ID conditions. For example, behaviors trained to interact with in-distribution (ID) pens can apply to interacting with a visually-OOD pencil. The key challenge lies in disambiguating which ID observations functionally correspond to the OOD observation for the task at hand. We propose that an expert can provide this OOD-to-ID functional correspondence. Thus, instead of collecting new demonstrations and re-training at every OOD encounter, our method: (1) detects the need for feedback by first checking if current observations are OOD and then identifying whether the most similar training observations show divergent behaviors, (2) solicits functional correspondence feedback to disambiguate between those behaviors, and (3) intervenes on the OOD observations with the functionally corresponding ID observations to perform deployment-time generalization. We validate our method across diverse real-world robotic manipulation tasks with a Franka Panda robotic manipulator. Our results show that test-time functional correspondences can improve the generalization of a vision-based diffusion policy to OOD objects and environment conditions with low feedback.

==> sections/intro.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width = \textwidth]{example-image-a}
    \caption{We present our method that leverages functional correspondences between deployment and training conditions, to improve policy performance under OOD Conditions}
    \label{teaser_figure}
\end{figure}


\section{Introduction}
\label{sec:intro}

% * Motivate the problem that you are trying to solve - why is it important?.
An overarching goal for robot learning has been to enable robots to generalize in unseen environments. Recently pre-training on internet-scale data has unlocked similar generalization capabilities in areas of computer vision and NLP. This advancement has provided new impetus to roboticists across the world to pre-train end-to-end imitation learning policies with large scale robotics datasets to attain generalization. 

% * Why is this problem hard?  Explain at a *high level* why current approaches (or other simple solutions) do not solve the problem.
However, unlike the vision and language domains the data for robot learning is not readily available. Collecting robot data involves repeated and meticulous interaction with the world through intricate tele-operation interfaces. This makes robotics data acquisition time and resource intensive. Years worth of effort from expert teleoperators have resulted in datasets, which are orders of magnitude smaller than vision and language datasets.

Although we lack the scale in terms of the data, recently we have made strides of improvement in the modeling choices as well. Recent end-to-end policy architectures have shown impressive capabilities at modeling complex multi-modal low level in-distribution behavior. 

Thus, the question that we ask in this work, is that is there a way to effectively re-use the skills that we already have acquired in in-distribution conditions to novel out-of-distribution conditions? 

% * Describe your ""key idea"" and give some intuition for why it should work

In order to generalize to conditions outside of your training distribution, we need an auxiliary source of information that facilitates knowledge transfer from in-distribution to out-of-distribution conditions. We hypothesize that  establishing functional correspondence across ID and OOD scenes unlocks this knowledge transfer for learning based robot policies.

Example of pens and pencils.

% * Outline your solution

Based on this insight, we present our method that queries the human knowledge about these high-level functional correspondences, and then uses these correspondences to steer a diffusion policy through OOD conditions. Detect OOD, if OOD semantic reasoning in the functional feature space, detect multi-modality in the final filtered features, ask user for clarification.

% * Describe key results
We evaluate our method on two real-world tasks of varying complexity, where we introduce OODness through novel objects and environments. Our method upholds task success rate better than the baselines, while being efficient at seeking expert feedback.

% * Summarize your contribution
In summary, in this work we test the how far we can take the idea of leveraging functional correspondences for zero shot behavior transfer.
we present a novel method that leverages functional correspondences to transfer behaviors from ID to OOD. It also serves as a recipe to leverage functional correspondences for zero-shot behavior transfer, where functional correspondences can come from anywhere. In our method we use an expert.

Our results show that with expert-guided functional correspondences transcends  generalization capabilities to objects from different semantic categories. 


% Other approaches train on diverse data, and more expressive modeling choices. 

% While the most naive thing to do in-order to recover from OOD conditions is to recollect demonstrations in OOD conditions and retrain, however there are some problems. \pranay{READ OTHER PAPERS TO TALK ABOUT THESE PROBLEMS}







% In order to function in unseen conditions, we need an auxiliary source of information connecting the unseen world to what we have seen before. Making this sort of a connection allows us to reuse the skills that we already possess in the new environment. 


% We largely bifurcate the OOD conditions into two large categories, semantic and behavioral. For behavioural we need new demonstrations. But semantic OOD conditions, lead to failure because the policy does not capture functionally task relevant correspondences between data. 
% Define functional task-relevant correspondences. We can leverage these correspondences to find functionally similar training data, and can intervene on the OOD test conditions using the corresponding training samples to uphold performance. Give an example.





